Extending Partial Representations of Proper and Unit Interval Graphs

The recently introduced problem of extending partial interval representations asks, for an interval graph with some intervals pre-drawn by the input, whether the partial representation can be extended to a representation of the entire graph. In this paper, we give a linear-time algorithm for extending proper interval representations and an almost quadratic-time algorithm for extending unit interval representations. We also introduce the more general problem of bounded representations of unit interval graphs, where the input constrains the positions of some intervals by lower and upper bounds. We show that this problem is NP-complete for disconnected input graphs and give a polynomial-time algorithm for the special class of instances, where the ordering of the connected components of the input graph along the real line is prescribed. This includes the case of partial representation extension. The hardness result sharply contrasts the recent polynomial-time algorithm for bounded representations of proper interval graphs [Balko et al. ISAAC'13]. So unless $\text{P} = \text{NP}$, proper and unit interval representations have vastly different structure. This explains why partial representation extension problems for these different types of representations require substantially different techniques.

==> simultaneous_representations.tex <==
\section{Simultaneous Representations} \label{sec:simrep}

Let $G_1,\dots,G_k$ be graphs having $V(G_i) \cap V(G_j) = I$ for each $i \ne j$. The
$\simrep(\calC)$ problem asks whether there exists representations $\calR_1,\dots,\calR_k$ of
$G_1,\dots,G_k$ (of class $\calC$) which assign the same sets to the vertices of $I$. This problem
was considered in~\cite{simultaneous_interval_graphs} and its relations to the partial
representation extension were discussed in~\cite{kkv}.

Let us consider the problems $\simrep(\pint)$ and $\simrep(\uint)$ which were not considered before.
Similarly to the partial representation problem, these two classes behave differently when
simultaneous representations are considered. We believe that the techniques used in this paper can
be applied to these simultaneous representations problems and they seem to be an interesting direction
for a future research. To show this, we solve a special case of $\simrep$ in which all graphs
$G_1,\dots,G_k$ are connected.

We start by pruning the graphs. If $u,v \in V(G_i)$, $u$ and $v$ are indistinguishable in $G_i$ and
$u \notin I$, we remove $u$ from $G_i$ (and later in $\calR_i$ we represent $u$ and $v$ by the same
interval). We repeat this until no such pair $u,v$ can be found in any graph, so if two vertices are
indistinguishable, they both belong to $I$. This can be done in time $\O(n+m)$ (for example, using
orderings $<$ from Corneil et al.~\cite{uint_corneil}).  For the rest of the section, we suppose
that the graphs are pruned.  We note that two vertices can be indistinguishable in one graph but can
be distinguishable in other graph.

First, we show a lemma concerning simultaneous orderings $\wlt_1,\dots,\wlt_k$.

\begin{lemma} \label{lem:sim_ordering}
If $G_1,\dots,G_k$ are connected and simultaneous representations $\calR'_1,\dots,\calR'_k$ exist,
then we can construct in $\O(n+m)$ simultaneous linear orderings $\wlt_1,\dots,\wlt_k$ of
$G_1,\dots,G_k$ such that there exist simultaneous representations $\calR_1,\dots,\calR_k$ in the
orderings $\wlt_1,\dots,\wlt_k$.
\end{lemma}

\begin{proof}
We start by computing left-to-right orders $<_1,\dots,<_k$ for each graph, using the algorithm of
Corneil et al.~\cite{uint_corneil}. Recall that each order is uniquely determined up to complete
reversal and reordering of the groups of indistinguishable vertices. So essentially, we have two
possibilities for each graph. To produce $\wlt_1,\dots,\wlt_k$, we need to find for each graph
whether to take the order $<_i$ or its reversal, so that the orders are the same on $I$.

Two orders $<_i$ and $<_j$ are \emph{equivalent on $I$} if for every $u,v \in I$ is $u <_j v$ if and
only if $u <_i v$. We process $<_1,\dots,<_k$ one-by-one. After processing $<_i$, we produce
$<'_1,\dots,<'_i$ which are pairwise equivalent on $I$. We first start with $<_1$ and keep it as it
is, putting $<'_1 = <_1$.  Now suppose that we have already processed $<'_1,<'_2,\dots,<'_{i-1}$ and
want to add $<_i$ to it.  We test this for both $<_i$ and its reversal (in the following, we
describe it just for $<_i$).

First we check $<_i$ from left to right whether its order of $I$ in compatible with
$<'_1,\dots,<'_{i-1}$. If we find a pair $u,v \in I$ such that $u <'_j v$ and $v <_i u$ for some $j
< i$, the order $<_i$ cannot be used. If neither $<_i$ or its reversal can be used, the construction
fails (which, as we show later, gives a contradiction with the assumptions). If $<_i$ can be used,
we create $<'_i$ from $<_i$ by additionally putting $u <'_i v$ if $u,v \in I$ and $u <'_j v$ for
some $j < i$. Then, we modify each $<'_1,\dots,<'_{i-1}$ according to $<'_i$, by putting $u <'_j v$
for each $u <'_i v$, $u,v \in H$. So, we obtain compatible orders $<'_1,\dots,<'_i$.

Let $\wlt'_1,\dots,\wlt'k$ be the representations of $\calR'_1,\dots,\calR'_k$ which exist by the
assumption of the lemma. We prove by induction on the number of the steps that the produced
orderings $<'_1,\dots,<'_i$ are extended by $\wlt'_1,\dots,\wlt'_i$ (or possibly by their complete
reversals). For the first step, $\wlt'_1$ or its reversal has to extend $<_1$ (so we possible
reverse $\calR'_1,\dots,\calR'_k$).

When $<_i$ is processed, by induction hypothesis $\wlt'_1,\dots,\wlt'_{i-1}$ extend
$<'_1,\dots,<'_{i-1}$. Now, suppose that the above procedure fails for $<_i$. Since both $<_i$ and
its reversal were rejected, then there exist $u,v,u',v' \in I$ such that $u <'_j v$, $u' <'_{j'}
v'$, $v <_i u$ and $u' <_i v'$. But since $\wlt'_i$ extends $<_i$ or its reversal (by
Lemma~\ref{pint_ordering}), then either $v \wlt'_i u$ or $u' \wlt'_i v'$ which makes $\wlt'_i$
incompatible with either $\wlt'_j$ or $\wlt'_{j'}$, so it contradicts existence of the
representations $\calR_1,\dots,\calR_k$.

The minimality means the following if $u,v \in I$ and $u <'_i v$, then $u$ is on the
left of $v$ for each simultaneous representations $\calR_1,\dots,\calR_k$ (up to complete reversal of
these simultaneous representations).

\end{proof}


\begin{proposition}
If $G_1,\dots,G_k$ are connected, then $\simrep(\pint)$ can be solved in time $\O(n+m)$ and
$\simrep(\uint)$ can be solved in polynomial-time using linear programming, where $n$ is the total
number of vertices and $m$ is the total number of edges in all graphs $G_i$.
\end{proposition}

\begin{proof}
We construct the common orderings $\wlt_1,\dots,\wlt_k$ using Lemma~\ref{lem:sim_ordering}.
Now, for proper interval graphs, these compatible orders are already a sufficient condition, and we
can use it to construct simultaneous representations. For unit interval graphs, there are additional
length conditions. To deal with them, we can apply a similar linear program as in
Subsection~\ref{subsec:lp_approach}.

Let $v^\alpha_1 \wlt_\alpha \dots \wlt_\alpha v^\alpha_{k_\alpha}$ be the ordered vertices of
$G_\alpha$, so $|G_\alpha| = k_\alpha$.  We solve the following linear program for variables
$\ell^\alpha_i$:

\begin{alignat}{2}
\ell^\alpha_i &\le \ell^\alpha_{i+1},&\qquad&\forall \alpha=1,\dots,k, \forall i=1,\dots,k_\alpha-1
																				\label{simrep_ordering}\\
\ell^\alpha_i &\ge \ell^\alpha_j - 1,&&
	\forall v^\alpha_iv^\alpha_j \in E(G_\alpha), v^\alpha_i \wlt_\alpha v^\alpha_j, \label{simrep_edges}\\
\ell^\alpha_i + \eps &\le \ell^\alpha_j -1,&&
	\forall v^\alpha_iv^\alpha_j \notin E(G_\alpha), v^\alpha_i \wlt_\alpha v^\alpha_j.	\label{simrep_nonedges}\\
\ell^\alpha_i &= \ell^\beta_j,&& \forall \alpha \ne \beta, v^\alpha_i = v^\beta_j. \label{simrep_condition}
\end{alignat}

Here, the constraints~(\ref{simrep_ordering}) force the orderings $\wlt_1,\dots,\wlt_k$. The
constraints~(\ref{simrep_edges}) and~(\ref{simrep_nonedges}) force $\calR_1,\dots,\calR_k$ to be
representations of $G_1,\dots,G_k$. Finally, the constraints~(\ref{simrep_condition}) force the
representations $\calR_1,\dots,\calR_k$ to be simultaneous. Since the constructed orderings
$\wlt_1,\dots,\wlt_k$ are correct, this linear program solves the simultaneous representations.\qed
\end{proof}



